First measurement of high-energy reactor antineutrinos at Daya Bay

This Letter reports the first measurement of high-energy reactor antineutrinos at Daya Bay, with nearly 9000 inverse beta decay candidates in the prompt energy region of 8-12~MeV observed over 1958 days of data collection. A multivariate analysis is used to separate 2500 signal events from background statistically. The hypothesis of no reactor antineutrinos with neutrino energy above 10~MeV is rejected with a significance of 6.2 standard deviations. A 29\% antineutrino flux deficit in the prompt energy region of 8-11~MeV is observed compared to a recent model prediction. We provide the unfolded antineutrino spectrum above 7 MeV as a data-based reference for other experiments. This result provides the first direct observation of the production of antineutrinos from several high-$Q_{\beta}$ isotopes in commercial reactors.

==> First measurement of high-energy reactor antineutrinos at Daya Bay/PhysRev.tex <==
%%% Generation information for this file
%%% Mon Mar  7 08:35:00 2022
%%% /Users/djaffe/Documents/Reactor/work/trunk/NuWa-trunk/dybgaudi/Documentation/AuthorList_SAVE/2021_HighEnergyReactorAntineutrinos
%%% ../AuthGen.py dyb_collabotion_list_20210201.xls 20210201 -1 TRUE 
\newcommand{\IHEP}{\affiliation{Institute~of~High~Energy~Physics, Beijing}}
\newcommand{\Wisconsin}{\affiliation{University~of~Wisconsin, Madison, Wisconsin 53706}}
\newcommand{\Yale}{\affiliation{Wright~Laboratory and Department~of~Physics, Yale~University, New~Haven, Connecticut 06520}} %%%% 20170227 add Wright Lab
\newcommand{\BNL}{\affiliation{Brookhaven~National~Laboratory, Upton, New York 11973}}
\newcommand{\NTU}{\affiliation{Department of Physics, National~Taiwan~University, Taipei}}
\newcommand{\NUU}{\affiliation{National~United~University, Miao-Li}}
\newcommand{\Dubna}{\affiliation{Joint~Institute~for~Nuclear~Research, Dubna, Moscow~Region}}
\newcommand{\CalTech}{\affiliation{California~Institute~of~Technology, Pasadena, California 91125}}
\newcommand{\CUHK}{\affiliation{Chinese~University~of~Hong~Kong, Hong~Kong}}
\newcommand{\NCTU}{\affiliation{Institute~of~Physics, National~Chiao-Tung~University, Hsinchu}}
\newcommand{\NJU}{\affiliation{Nanjing~University, Nanjing}}
\newcommand{\TsingHua}{\affiliation{Department~of~Engineering~Physics, Tsinghua~University, Beijing}}
\newcommand{\SZU}{\affiliation{Shenzhen~University, Shenzhen}}
\newcommand{\NCEPU}{\affiliation{North~China~Electric~Power~University, Beijing}}
\newcommand{\Siena}{\affiliation{Siena~College, Loudonville, New York  12211}}
\newcommand{\IIT}{\affiliation{Department of Physics, Illinois~Institute~of~Technology, Chicago, Illinois  60616}}
\newcommand{\LBNL}{\affiliation{Lawrence~Berkeley~National~Laboratory, Berkeley, California 94720}}
\newcommand{\UIUC}{\affiliation{Department of Physics, University~of~Illinois~at~Urbana-Champaign, Urbana, Illinois 61801}}
\newcommand{\SJTU}{\affiliation{Department of Physics and Astronomy, Shanghai Jiao Tong University, Shanghai Laboratory for Particle Physics and Cosmology, Shanghai}}
\newcommand{\BNU}{\affiliation{Beijing~Normal~University, Beijing}}
\newcommand{\WM}{\affiliation{College~of~William~and~Mary, Williamsburg, Virginia  23187}}
\newcommand{\Princeton}{\affiliation{Joseph Henry Laboratories, Princeton~University, Princeton, New~Jersey 08544}}
\newcommand{\VirginiaTech}{\affiliation{Center for Neutrino Physics, Virginia~Tech, Blacksburg, Virginia  24061}}
\newcommand{\CIAE}{\affiliation{China~Institute~of~Atomic~Energy, Beijing}}
\newcommand{\SDU}{\affiliation{Shandong~University, Jinan}}
\newcommand{\NanKai}{\affiliation{School of Physics, Nankai~University, Tianjin}}
\newcommand{\UC}{\affiliation{Department of Physics, University~of~Cincinnati, Cincinnati, Ohio 45221}}
\newcommand{\DGUT}{\affiliation{Dongguan~University~of~Technology, Dongguan}}
\newcommand{\XJTU}{\affiliation{Department of Nuclear Science and Technology, School of Energy and Power Engineering, Xi'an Jiaotong University, Xi'an}}%%updated 20161215 {Xi'an Jiaotong University, Xi'an}}
\newcommand{\UCB}{\affiliation{Department of Physics, University~of~California, Berkeley, California  94720}}
\newcommand{\HKU}{\affiliation{Department of Physics, The~University~of~Hong~Kong, Pokfulam, Hong~Kong}}
\newcommand{\Charles}{\affiliation{Charles~University, Faculty~of~Mathematics~and~Physics, Prague}} %updated20140819
\newcommand{\USTC}{\affiliation{University~of~Science~and~Technology~of~China, Hefei}}
\newcommand{\TempleUniversity}{\affiliation{Department~of~Physics, College~of~Science~and~Technology, Temple~University, Philadelphia, Pennsylvania  19122}}
\newcommand{\CGNPG}{\affiliation{China General Nuclear Power Group, Shenzhen}}% update 20170729 add city. updated 20140724 China~Guangdong~Nuclear~Power~Group, Shenzhen}}
\newcommand{\NUDT}{\affiliation{College of Electronic Science and Engineering, National University of Defense Technology, Changsha}} % added 20140111
\newcommand{\IowaState}{\affiliation{Iowa~State~University, Ames, Iowa  50011}}
\newcommand{\ZSU}{\affiliation{Sun Yat-Sen (Zhongshan) University, Guangzhou}}
\newcommand{\CQU}{\affiliation{Chongqing University, Chongqing}} % add 20150417
\newcommand{\BCC}{\altaffiliation[Now at ]{Department of Chemistry and Chemical Technology, Bronx Community College, Bronx, New York  10453}} % add 20160311 for Sunej's 'now at'

\newcommand{\UCI}{\affiliation{Department of Physics and Astronomy, University of California, Irvine, California 92697}} %20190209 for Pedro's new digs
\newcommand{\GXU}{\affiliation{Guangxi University, No.100 Daxue East Road, Nanning}} % added 20201208 ,530004, China
\author{F.~P.~An}\ZSU
\author{W.~D.~Bai}\ZSU
\author{A.~B.~Balantekin}\Wisconsin
\author{M.~Bishai}\BNL
\author{S.~Blyth}\NTU
\author{G.~F.~Cao}\IHEP
\author{J.~Cao}\IHEP
\author{J.~F.~Chang}\IHEP
\author{Y.~Chang}\NUU
\author{H.~S.~Chen}\IHEP
\author{H.~Y.~Chen}\TsingHua
\author{S.~M.~Chen}\TsingHua
\author{Y.~Chen}\SZU\ZSU
\author{Y.~X.~Chen}\NCEPU
\author{J.~Cheng}\NCEPU
\author{Z.~K.~Cheng}\ZSU
\author{J.~J.~Cherwinka}\Wisconsin
\author{M.~C.~Chu}\CUHK
\author{J.~P.~Cummings}\Siena
\author{O.~Dalager}\UCI
\author{F.~S.~Deng}\USTC
\author{Y.~Y.~Ding}\IHEP
\author{M.~V.~Diwan}\BNL
\author{T.~Dohnal}\Charles
\author{D.~Dolzhikov}\Dubna
\author{J.~Dove}\UIUC
\author{D.~A.~Dwyer}\LBNL
\author{J.~P.~Gallo}\IIT
\author{M.~Gonchar}\Dubna
\author{G.~H.~Gong}\TsingHua
\author{H.~Gong}\TsingHua
\author{W.~Q.~Gu}\BNL
\author{J.~Y.~Guo}\ZSU
\author{L.~Guo}\TsingHua
\author{X.~H.~Guo}\BNU
\author{Y.~H.~Guo}\XJTU
\author{Z.~Guo}\TsingHua
\author{R.~W.~Hackenburg}\BNL
\author{S.~Hans}\BCC\BNL
\author{M.~He}\IHEP
\author{K.~M.~Heeger}\Yale
\author{Y.~K.~Heng}\IHEP
\author{Y.~K.~Hor}\ZSU
\author{Y.~B.~Hsiung}\NTU
\author{B.~Z.~Hu}\NTU
\author{J.~R.~Hu}\IHEP
\author{T.~Hu}\IHEP
\author{Z.~J.~Hu}\ZSU
\author{H.~X.~Huang}\CIAE
\author{J.~H.~Huang}\IHEP
\author{X.~T.~Huang}\SDU
\author{Y.~B.~Huang}\GXU
\author{P.~Huber}\VirginiaTech
\author{D.~E.~Jaffe}\BNL
\author{K.~L.~Jen}\NCTU
\author{X.~L.~Ji}\IHEP
\author{X.~P.~Ji}\BNL
\author{R.~A.~Johnson}\UC
\author{D.~Jones}\TempleUniversity
\author{L.~Kang}\DGUT
\author{S.~H.~Kettell}\BNL
\author{S.~Kohn}\UCB
\author{M.~Kramer}\LBNL\UCB
\author{T.~J.~Langford}\Yale
\author{J.~Lee}\LBNL
\author{J.~H.~C.~Lee}\HKU
\author{R.~T.~Lei}\DGUT
\author{R.~Leitner}\Charles
\author{J.~K.~C.~Leung}\HKU
\author{F.~Li}\IHEP
\author{H.~L.~Li}\IHEP
\author{J.~J.~Li}\TsingHua
\author{Q.~J.~Li}\IHEP
\author{R.~H.~Li}\IHEP
\author{S.~Li}\DGUT
\author{S.~C.~Li}\VirginiaTech
\author{W.~D.~Li}\IHEP
\author{X.~N.~Li}\IHEP
\author{X.~Q.~Li}\NanKai
\author{Y.~F.~Li}\IHEP
\author{Z.~B.~Li}\ZSU
\author{H.~Liang}\USTC
\author{C.~J.~Lin}\LBNL
\author{G.~L.~Lin}\NCTU
\author{S.~Lin}\DGUT
\author{J.~J.~Ling}\ZSU
\author{J.~M.~Link}\VirginiaTech
\author{L.~Littenberg}\BNL
\author{B.~R.~Littlejohn}\IIT
\author{J.~C.~Liu}\IHEP
\author{J.~L.~Liu}\SJTU
\author{J.~X.~Liu}\IHEP
\author{C.~Lu}\Princeton
\author{H.~Q.~Lu}\IHEP
\author{K.~B.~Luk}\UCB\LBNL
\author{B.~Z.~Ma}\SDU
\author{X.~B.~Ma}\NCEPU
\author{X.~Y.~Ma}\IHEP
\author{Y.~Q.~Ma}\IHEP
\author{R.~C.~Mandujano}\UCI
\author{C.~Marshall}\LBNL
\author{K.~T.~McDonald}\Princeton
\author{R.~D.~McKeown}\CalTech\WM
\author{Y.~Meng}\SJTU
\author{J.~Napolitano}\TempleUniversity
\author{D.~Naumov}\Dubna
\author{E.~Naumova}\Dubna
\author{T.~M.~T.~Nguyen}\NCTU
\author{J.~P.~Ochoa-Ricoux}\UCI
\author{A.~Olshevskiy}\Dubna
\author{H.-R.~Pan}\NTU
\author{J.~Park}\VirginiaTech
\author{S.~Patton}\LBNL
\author{J.~C.~Peng}\UIUC
\author{C.~S.~J.~Pun}\HKU
\author{F.~Z.~Qi}\IHEP
\author{M.~Qi}\NJU
\author{X.~Qian}\BNL
\author{N.~Raper}\ZSU
\author{J.~Ren}\CIAE
\author{C.~Morales~Reveco}\UCI
\author{R.~Rosero}\BNL
\author{B.~Roskovec}\Charles
\author{X.~C.~Ruan}\CIAE
\author{H.~Steiner}\UCB\LBNL
\author{J.~L.~Sun}\CGNPG
\author{T.~Tmej}\Charles
\author{K.~Treskov}\Dubna
\author{W.-H.~Tse}\CUHK
\author{C.~E.~Tull}\LBNL
\author{B.~Viren}\BNL
\author{V.~Vorobel}\Charles
\author{C.~H.~Wang}\NUU
\author{J.~Wang}\ZSU
\author{M.~Wang}\SDU
\author{N.~Y.~Wang}\BNU
\author{R.~G.~Wang}\IHEP
\author{W.~Wang}\ZSU\WM
\author{X.~Wang}\NUDT
\author{Y.~Wang}\NJU
\author{Y.~F.~Wang}\IHEP
\author{Z.~Wang}\IHEP
\author{Z.~Wang}\TsingHua
\author{Z.~M.~Wang}\IHEP
\author{H.~Y.~Wei}\BNL
\author{L.~H.~Wei}\IHEP
\author{L.~J.~Wen}\IHEP
\author{K.~Whisnant}\IowaState
\author{C.~G.~White}\IIT
\author{H.~L.~H.~Wong}\UCB\LBNL
\author{E.~Worcester}\BNL
\author{D.~R.~Wu}\IHEP
\author{Q.~Wu}\SDU
\author{W.~J.~Wu}\IHEP
\author{D.~M.~Xia}\CQU
\author{Z.~Q.~Xie}\IHEP
\author{Z.~Z.~Xing}\IHEP
\author{H.~K.~Xu}\IHEP
\author{J.~L.~Xu}\IHEP
\author{T.~Xu}\TsingHua
\author{T.~Xue}\TsingHua
\author{C.~G.~Yang}\IHEP
\author{L.~Yang}\DGUT
\author{Y.~Z.~Yang}\TsingHua
\author{H.~F.~Yao}\IHEP
\author{M.~Ye}\IHEP
\author{M.~Yeh}\BNL
\author{B.~L.~Young}\IowaState
\author{H.~Z.~Yu}\ZSU
\author{Z.~Y.~Yu}\IHEP
\author{B.~B.~Yue}\ZSU
\author{V.~Zavadskyi}\Dubna
\author{S.~Zeng}\IHEP
\author{Y.~Zeng}\ZSU
\author{L.~Zhan}\IHEP
\author{C.~Zhang}\BNL
\author{F.~Y.~Zhang}\SJTU
\author{H.~H.~Zhang}\ZSU
\author{J.~L.~Zhang}\NJU
\author{J.~W.~Zhang}\IHEP
\author{Q.~M.~Zhang}\XJTU
\author{S.~Q.~Zhang}\ZSU
\author{X.~T.~Zhang}\IHEP
\author{Y.~M.~Zhang}\ZSU
\author{Y.~X.~Zhang}\CGNPG
\author{Y.~Y.~Zhang}\SJTU
\author{Z.~J.~Zhang}\DGUT
\author{Z.~P.~Zhang}\USTC
\author{Z.~Y.~Zhang}\IHEP
\author{J.~Zhao}\IHEP
\author{R.~Z.~Zhao}\IHEP
\author{L.~Zhou}\IHEP
\author{H.~L.~Zhuang}\IHEP
\author{J.~H.~Zou}\IHEP
